CoReQA: Uncovering Potentials of Language Models in Code Repository Question Answering

Large language models that enhance software development tasks, such as code generation, code completion, and code question answering (QA), have been extensively studied in both academia and the industry. The models are integrated into popular intelligent IDEs like JetBrains and Cursor. Current benchmarks for evaluating models' code comprehension capabilities primarily focus on code generation or completion, often neglecting QA, which is a crucial aspect of understanding code. Existing code QA benchmarks are derived from code comments with predefined patterns (e.g., CodeQA) or focus on specific domains, such as education (e.g., CS1QA). These benchmarks fail to capture the real-world complexity of software engineering and user requirements for understanding code repositories. To address this gap, we introduce CoReQA, a benchmark for Code Repository-level question answering, constructed from GitHub issues and comments from 176 popular repositories across four programming languages. Since questions and answers may include both natural language and code snippets, traditional evaluation metrics such as BLEU are inadequate for assessing repository-level QA performance. Thus, we provide an LLM-as-a-judge framework to evaluate QA performance from five aspects. Based on CoReQA, we evaluate the performance of three baselines, including two short-context models using generic retrieval strategies and one long-context model that utilizes the entire repository context. Evaluation results show that state-of-the-art proprietary and long-context models struggle to address repository-level questions effectively. Our analysis highlights the limitations of language models in assisting developers in understanding repositories and suggests future directions for improving repository comprehension systems through effective context retrieval methodologies.

==> CaseStudy.tex <==
\section{Case Study}
We may provide case study of our benchmark to compare the performance  with some industry work.


==> Introduction.tex <==
\section{Introduction}


% \textbf{abstract ddl: 26 July 2024. 
% submission: 2 Aug 2024}

% \textbf{Target}: ICSE'2025 - Research Track - \textit{Efficacy measurement beyond traditional metrics (e.g., accuracy, BLEU, etc.) \textbf{OR}  AI-enabled recommender systems for automated SE}



% 1. SWE only involve bug report and feature request issues. Researchers may involve other questions to understand the codebase, enhance the functionality of the code base or apply the codebase to satisfy their owen features. Maybe we provide a propotion of QA/bugrepot or QA/feature request

% 1. Motivations: 
% 1.1 Existing works/benchmark 


% 2. Challenges/Limitations of existing work:
 
% 3. Solutions: 




% propose background 

Large language models (LLMs)~\cite{deepseek2024, chatgpt2024, claude2024, gemini2024} have exhibited exceptional proficiency in interpreting natural language semantics.
%
Leveraging the inherent analogy between code and natural language—where both are fundamentally composed of structured word sequences—researchers have effectively broadened the scope of large language models to include comprehension of code semantics  (Code-LLMs)~\cite{deepseek2024}.
%
By augmenting the training corpus with code examples, Code-LLMs~\cite{chatgpt2024,guo2024deepseek, cursor2024, nam2024using,bai2023qwen} are now adept at supporting a variety of code-centric tasks. 
%
These tasks encompass but are not limited to, code completion~\cite{zhang2023repocoder,li2023cctest,nie2023learning}, question answering~\cite{budler2023review, omar2023chatgpt, hu2023tifa} and the remediation of software defects~\cite{sobania2023analysis, ni2020analyzing, drain2021generating}, thereby providing a robust toolkit to enhance the development process.%


\begin{figure}[t!]
    \centering
    \includegraphics[width=1\linewidth]{Figs/ShowCase.pdf}
    \caption{A question-answer pair from a sample GitHub issue and comments.}
    \label{fig:showcase}
\end{figure}



% introduce related benchmarks
To evaluate the effectiveness of Code-LLMs, benchmarks~\cite{yu2024codereval,chen2021humaneval,ding2023crosscodeeval,jimenez2023swe,zhang2023repocoder} have been constructed to assess the performance of LLMs on coding tasks. 
%
Initially, benchmarks typically focused on straightforward coding tasks that do not require extensive contextual information and can be effectively addressed with a single task or code file. 
%
% For example, XXX. 
%
However, in real-world scenarios, coding tasks tend to be more complex. 
%
For instance, when tackling a function-level code-completion task, it is often beneficial to refer to relevant functions~\cite{yu2024codereval, jimenez2023swe} imported in the current code file. 
%to generate the required functionality more effectively and concisely. 
By doing so, developers can generate the desired functionality in a more efficient and concise manner.
%
\jialiang{add reference here}
Consequently, cross-file benchmarks have been introduced to better reflect these real-world complexities~\cite{??}.
%
% XXX


% propose requirements and limitation of existing works
Existing benchmarks~\cite{yu2024codereval, zhang2023repocoder, chen2021humaneval,zhang2024codeagent} primarily focus on program generation tasks, such as code generation and automated code completion.
%
Code generation~\cite{zhang2024codeagent, svyatkovskiy2020intellicode,le2022coderl} entails algorithmically creating source code from natural language descriptions, transforming code between different programming languages, or deriving code from API documentation. 
%
% This capability is typically encapsulated within interactive chatbot interfaces, which facilitate the translation of user-provided specifications into functional code segments, thereby streamlining the development process and enabling rapid prototyping.
%
% Conversely, 
Code completion is an essential feature within Integrated Development Environments (IDEs) like Cursor~\cite{cursor2024}, Copilot~\cite{GitHubCopilot}, and JetBrains~\cite{JetBrainsWebsite}, offering real-time suggestions for code snippets based on partial code or accompanying comments provided by developers. %
% By providing contextually relevant completions, code completion services enhance coding efficiency, reduce the likelihood of errors, and accelerate the software development lifecycle.
% For example, SWE-bench~\cite{jimenez2023swe} 
%
These benchmarks assess the functionality of generated code snippets using pre-designed unit tests~\cite{zhang2023repocoder, yu2024codereval} or the operating system's \texttt{patch} program~\cite{jimenez2023swe}.
%





While code generation benchmarks have been thoroughly explored, there is a conspicuous dearth of benchmarks addressing question-answering (QA) scenarios that are pivotal to contemporary code assistant tools, such as  Copilot, Cursor, or Phorm.
%
In contrast to code generation tasks that focus on producing executable code snippets, question answering in code assistance necessitates responding to diverse user inquiries. 
%
These may encompass queries related to programming techniques, searches for problem-solving strategies, guidance on adapting functionalities to individual requirements, elucidation of specific code definitions, and more.
%



Current Code QA benchmarks~\cite{sahu2024codequeries} are limited in scope, often accommodating only straightforward answer formats, such as binary responses or brief phrases, and tackling simplistic content, focusing on isolated code snippets or single files. 
%
However, real-world scenarios frequently demand comprehension of entire projects or clarification of inter-function dependencies. Users' queries in these contexts expect comprehensive responses that blend natural language explanations with pertinent code examples. 
%
The advent of advanced QA features, exemplified by Cursor's side chat, underscores the necessity for a robust benchmark to gauge the efficacy of these QA engines.


To address this deficiency, we introduce RepoQA-bench, a benchmark designed for repository-level question answering. 
%
RepoQA-bench aims to simulate the complexity and diversity of real-world inquiries, thereby facilitating a more accurate evaluation of QA systems' capabilities within the context of extensive code repositories.
%
%
To establish RepoQA-bench as a credible benchmark, we initiate the process by devising an issue-based query generation framework. 
%
This framework ensures that queries mirror developers' authentic, day-to-day demands, thereby enhancing our benchmark's practical relevance. 
%
\jialiang{FIXME:Haven't implemented in this paper, remove or not?
Acknowledging that repository-scale questions often necessitate understanding interconnected code elements, we implement an automated retrieval mechanism to gather relevant cross-file content. 
}

%
% This is further augmented by meticulous manual inspections to uphold the benchmark's precision and relevancy.
%
The creation of reliable reference answers is another pivotal aspect. 
%
\jialiang{We employ prompt engineering methodologies to derive and rewrite reference answers from issue comments.}
% We employ prompt engineering methodologies that integrate retrieval contextual code chunks to produce these references. 

%
\jialiang{FIXME:No vetting now.
Manual vetting is then applied to filter out ambiguous or misleading questions, thus safeguarding the benchmark's integrity.
}
%
Fig.~\ref{fig:showcase} shows a question-answer pair from a sample GitHub issue and comments in RepoQA-bench.
%
The questions in RepoQA-bench are sourced from GitHub issues, and answers are generated regarding positive comments on the issue.
%
A crucial challenge lies in evaluating the generated responses effectively. To overcome this, we accompany the RepoQA-bench with a comprehensive evaluation framework. 
%
This framework is designed to accommodate retrieval-augmented generation strategies. It assesses the system's ability to handle extended contexts, ensuring a thorough and fair appraisal of QA models underpinning complex code repositories.


Our major contributions are summarized as follows: 
\begin{itemize}
\item We introduce RepoQA, a benchmark for repository question answering constructed from GitHub repositories across various domains and programming languages. 
%
The questions in RepoQA-bench are derived from real-world user issues, with answers sourced from corresponding discussions and comments. 
%
% The benchmark is available at \url{}.
%
% RepoQA-bench includes cross-file context to effectively address questions and undergoes in-house human inspection to ensure the quality of the QA pairs.

\item We evaluate and compare state-of-the-art large language models (LLMs) on RepoQA-bench. 
%
Our evaluations include base LLMs with retrieval strategies and long-context LLMs that address cross-file challenges. 
%
Our experiments highlight that repository-level question answering remains challenging for LLMs, 
and precise context retrieval strategies are urgently needed to improve the models' performance in this area.
% and precise context significantly improves performance in this area.

\item We provide an automated framework to construct repository-level QA pairs and a novel evaluation infrastructure to assess the performance of generative models in addressing repository-level questions.

%


\end{itemize}
\jialiang{FIXME:
The raw data obtained in this study cannot be shared because of confidentiality agreements. We do not plan to open-source the code and data at this time. However, we have made all the prompts used in the paper publicly available so that other researchers can reproduce our results. Once we receive the necessary permissions, we will open-source all the code and data.
}
% We plan to make RepoQA-bench and all associated experimental results publicly accessible\footnote{We will provide our code here.} to support research and development in repository question answering.




\noindent\textbf{Roadmap.} 
The remainder of the paper is organized as follows: 
%
\S\ref{sec:background}  provides basic background on 
% LLM-based 
code comprehension and retrieval argument generation systems in this area. 
%
\S\ref{sec:repoqatask} clarifies the tasks for repository question answering.
%
\S\ref{sec:repoqa}  introduces the components of RepoQA-bench. 
%
\S\ref{sec:evaluation} presents the experimental settings and results of baseline models. 
%
\S\ref{sec:relatedwork} reviews related work.
%
\S\ref{sec:discussion} discusses threats to validity, ethical considerations, limitations, and future work.
%
\S\ref{sec:conclusion} concludes this work.





==> Preliminary.tex <==
\section{Background}
\label{sec:background}

In this section, we first introduce cross-file code comprehension. 
%
Then, we introduce retrieval argument generation.
%
% Finally, we will introduce related benchmarks.  



% \subsection{Cross-file code comprehension}
\subsection{LLM-based code comprehension}



In the software development scenario, 
% cross-file 
code comprehension~\cite{ben2018neural,porkolab2018codecompass,bertolotti2023fold2vec} proves indispensable, given the iterative dependencies among code elements that collectively enable intricate functionalities. 
%
For instance, to automatically append an optimal code segment~\cite{zhang2024codeagent, ding2023crosscodeeval, luo2024repoagent}, developers must grasp the roles of imported modules and discern between identically named functions belonging to different classes. 
%
Similarly, crafting an accurate pull request~\cite{jimenez2023swe} for a repository necessitates a clear grasp of requirements, alongside the aggregation of pertinent data, logs, and error messages.


Even with the advent of large language models~\cite{chatgpt2024,gemini2024,deepseek2024,claude2024}, effectively tackling cross-file code comprehension remains a substantial hurdle. 
%
Firstly, interpreting the intent~\cite{9001577,pearce2023build} behind cross-file requirements can prove inconsistent due to inherent ambiguity. 
%
Secondly, accurately retrieving all relevant information scattered across different files is a promising solution. 
%
Besides, constructing the appropriate context for these models to pinpoint the crux of the issue and formulate a resolution is a non-trivial endeavor.
%
This underscores the pressing need for advancements in models and methods that can adeptly navigate and comprehend the interconnectedness of code repositories.








\subsection{Retrieval Augmented Generation}

Retrieval-augmented generation (RAG) enhances natural language processing (NLP) by combining retrieval-based AI with generative models. 
%
RAG addresses the limitations of large language models (LLMs) that often lack access to real-time and comprehensive external information. 
%
By integrating a retriever component that fetches relevant documents or data from a large corpus with a generator component that synthesizes this information into coherent responses, RAG systems provide more accurate and contextually appropriate answers \cite{dong2022survey}. 
%
The retriever identifies the most relevant pieces of information based on the input query, and the generator uses this context to construct a detailed response \cite{ren2023retrieve, li2024matching}. 
%
This combination significantly enhances the utility of LLMs in applications requiring up-to-date and specific knowledge.



Implementing RAG particularly benefits academic search engines and code repository question-answering domains. 
%
For instance, in the context of code repositories, RAG can retrieve relevant code snippets from various files and generate comprehensive explanations or solutions, aiding in cross-file code comprehension \cite{luo2024repoagent, lee2022cs1qa}. 
%
The workflow involves processing a user query, retrieving pertinent documents, and generating a synthesized answer, ensuring that the response is both accurate and informative \cite{liu2021codeqa}. 
%
This approach not only improves the accuracy of responses but also leverages dynamic and external information that static models might miss, making RAG a crucial advancement in the field of NLP and software engineering \cite{jimenez2023swe, ding2023crosscodeeval, liu2021codeqa}.


\begin{comment}
    
\subsection{Statistical Comparison with Different Benchmarks}

\begin{table}[t]
\caption{Comparison of Related Benchmarks}
\label{tab:relatedbenchmarks}
\centering
\resizebox{0.95\columnwidth}{!}{%
\begin{tabular}{@{}lrcll@{}}
\toprule
\multicolumn{1}{c}{Benchmark} &
\multicolumn{1}{c}{Size} &
Scenario &
\multicolumn{1}{c}{Granularity} &
\multicolumn{1}{c}{Language} \\ \midrule
CoderEval~\cite{yu2024codereval}    & 460   & CG & Cross file  & Python, Java. \\
CodeAgent~\cite{zhang2024codeagent} & 101  & CG & Cross file  & Python.       \\
SWE-Bench~\cite{jimenez2023swe}     & 2,294    & CG & Cross file  & Python.       \\
HumanEval~\cite{chen2021humaneval}  & 164   & CG & Single file & Python.       \\
CrossCodeEval~\cite{ding2023crosscodeeval} &
\multicolumn{1}{r}{9,928} &
CC &
Cross file &
\begin{tabular}[c]{@{}l@{}}Python, C\#, \\ Java, TypeScript.\end{tabular} \\
CodeQueries~\cite{sahu2024codequeries}     & 52 & QA & Cross file  & Python.       \\
CodeQA~\cite{liu2021codeqa}     & 190k+ & QA & Single file & Java, Python. \\
CS1QA~\cite{lee2022cs1qa}       & 9,237 & QA & Single file & Python.\\
\hline
RepoQA         & XXX & QA   & Cross file            &   \begin{tabular}[c]{@{}l@{}}Python, Java, \\ TypeScript, Go.\end{tabular}             \\ \bottomrule
\multicolumn{5}{l}{QA: Question Answering; CG: Code Generation; CC: Code Completion}
\end{tabular}%
}
\end{table}



Table~\ref{tab:relatedbenchmarks} gives the statistics of code comprehension related benchmarks. 
%
Existing benchmarks either limited to sin
\end{comment}


==> Thread2Val.tex <==
\section{Thread To Validation}

==> introduction_v2.tex <==
\section{Introduction}
% overall background - LLMs --> codeLLM --> code QA
Large language models (LLMs)~\cite{deepseek2024, chatgpt2024, claude2024, gemini2024} demonstrate exceptional proficiency in understanding and processing natural language.
%
Recently, LLMs trained on extensive code datasets (Code-LLMs)~\cite{chatgpt2024,guo2024deepseek, cursor2024, nam2024using,bai2023qwen} have shown promising results in software engineering tasks.
These tasks include code completion~\cite{zhang2023repocoder,li2023cctest,nie2023learning}, code summarization~\cite{ahmed2022few} and bug fixing~\cite{sobania2023analysis, ni2020analyzing, drain2021generating}. 
% research senario: code QA

%
% question answering~\cite{budler2023review, omar2023chatgpt, hu2023tifa}
Related tasks encompass but are not limited to, code completion~\cite{zhang2023repocoder,li2023cctest,nie2023learning}, code summarization~\cite{ahmed2022few} and the remediation of software defects~\cite{sobania2023analysis, ni2020analyzing, drain2021generating}. 
% research senario: code QA 
With Code-LLMs applied to code plugins or tools within Integrated Development Environments (IDEs) like Cursor~\cite{cursor2024}, Copilot~\cite{GitHubCopilot}, and JetBrains~\cite{JetBrainsWebsite}, side-chat functionalities targeting code question answering (code QA) tasks have become increasingly important.
% TODO: code QA could enhance the programming productivity by xx%


%% related works & motivation
% the code QA benchmarks
To assess the effectiveness of code QA tasks, several recent works have introduced code QA datasets specifically for evaluation purposes~\cite{sahu2024codequeries, liu2021codeqa, lee2022cs1qa}.
% Several recent works have provided code QA datasets for evaluation purposes~\cite{sahu2024codequeries, liu2021codeqa, lee2022cs1qa}. 
Existing work on question-answering over code has primarily considered yes or no questions or method-level context~\cite{liu2021codeqa, bansal2021neural}, more recent work~\cite{sahu2024codequeries} has provided a code QA dataset for the file level.
%
However, there is no semantically rich question-answering benchmark for complex, large-scope questions in real-world scenarios, which often require comprehension of entire projects (i.e., repository-level) or clarification of inter-function dependencies. 
%
The responses to questions in these contexts are also expected to be comprehensive, blending natural language explanations with relevant code examples.
% repo-level benchmarks
Although there are benchmarks for repository-level code understanding tasks like bug fixing~\cite{jimenez2023swe} and code generation~\cite{yu2024codereval, jimenez2023swe}, the literature lacks a benchmark specifically for repository-level code QA.


% methodology 
To address this gap, we introduce RepoQA-bench, a benchmark designed for repository-level question answering. 
%
RepoQA-bench aims to simulate the complexity and diversity of real-world inquiries, thereby facilitating a more accurate evaluation of QA systems' capabilities within the context of extensive code repositories. 
% 
To establish RepoQA-bench as a credible benchmark, we initiate the process by devising an issue-based QA generation framework. 
% data collection
We collect real-world GitHub issues and compile a dataset of 1,563 QA pairs from 190 repositories across four programming languages.
% question construction
We utilize the advanced semantic analysis capabilities of LLMs to integrate the collected issue titles and descriptions, rewriting them into questions related to code repositories.
% answer construction
To create reliable reference answers, we select issue comments with at least three positive marks by different GitHub users, and generate  answers from these human-supported comments. 
% example
Fig.~\ref{fig:showcase} shows a question-answer pair from a sample GitHub issue and comments in RepoQA-bench. 
%
The questions in RepoQA-bench source from GitHub issues, and answers are generated regarding positive comments on the issue.
%
Our framework ensures that QA pairs mirror developers' authentic, day-to-day demands, thereby enhancing our benchmark's practical relevance.

\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.7\linewidth]{Figs/ShowCase.pdf}
    \caption{A question-answer pair from a sample GitHub issue and comments.}
    \label{fig:showcase}
\end{figure*}


% result
To assess the effectiveness of RepoQA-bench, we accompany the RepoQA-bench with a comprehensive evaluation framework. 
%
% The evaluation ramework leverages the LLM-as-a-judge approach, scoring different LLM models across four aspects: accuracy, completeness, relevance, and clarity.
The evaluation framework employs the LLM-as-a-judge approach~\cite{NEURIPSllmjudge, es2023ragas} for two key aspects: absolute quality evaluation assessing accuracy, completeness, relevance, and clarity, and pairwise comparison evaluation for direct inter-model performance assessment.
%
Specifically, we evaluate three state-of-the-art LLMs (GPT-4o~\cite{chatgpt2024}, Gemini-1.5~\cite{gemini2024}, and DeepSeek-V2~\cite{deepseek2024}) using RepoQA-bench dataset. 
Additionally, we evaluate these models performance with a basic retrieval-augmented generation (RAG) strategy, i.e., BM25~\cite{robertson2004simple}. 
Furthermore, we assess the performance of long-context model (Gemini-1.5) performance by using the entire repository information as context.
%
These models achieve limited success on the RepoQA-bench, with average scores of 6.37, 5.70, 7.33, and 8.09 out of 10 in accuracy, completeness, relevance, and clarity. 
Scores increase to 6.40, 5.74, 7.36, 8.11 in accuracy, completeness, relevance, and clarity with retrieved relevant context.
%
The RepoQA-bench is thus a challenging dataset that can be used for evaluating code QA tasks and can further help identify opportunities to improve the performance of code QA task.

% 3 contribution
Our major contributions are summarized as follows: 
\begin{itemize}
\item We provide an automated framework to construct repository-level QA pairs and a novel evaluation infrastructure to assess the performance of generative models in addressing repository-level questions.

\item We introduce RepoQA, a benchmark for repository question answering constructed from GitHub repositories across various domains and programming languages. 
%
The questions in RepoQA-bench are derived from real-world user issues, with answers sourced from corresponding discussions and comments. 
%
% The benchmark is available at \url{}.
%
% RepoQA-bench includes cross-file context to effectively address questions and undergoes in-house human inspection to ensure the quality of the QA pairs.

\item We evaluate and compare state-of-the-art LLMs on RepoQA-bench. 
%
Our evaluations include base LLMs with retrieval strategies and long-context LLMs that address cross-file challenges. 
%
Our experiments highlight that repository-level question answering task remains challenging for LLMs, 
and precise context retrieval strategies are urgently needed to improve the models' performance in this area.
% and precise context significantly improves performance in this area.


\end{itemize}
%
% Optional Roadmap


==> materials/RepoQA_Construction.tex <==
1. How to collect repo-qa-datasets from GitHub issue?
1.1 数据收集 
  1. 开源仓库选择
    1. 比较活跃 (处于某个语言的 Top500 & issue 数量 > 200) 
    TODO: 明确下哪些语言：Go, python, C, C++, Java, Kotlin, Rust, JavaScript, TypeScript
    2. 比较新（尽量\textit{没有被训练过}，created_at >= '2022-01-01'）
    3. 仓库大小合理（Toke衡量，token 数量太多的仓库无法评估 Longcontext 产品）
  2. Crawl: Issues with all comments, 数据格式参考如下链接(这里暂时保留所有原始数据)
    1. comments: https://api.github.com/repos/huggingface/peft/issues/39/comments
1.2 数据清洗
  1. 筛选出包含正向 comments 的 issue（icons：大拇指/点赞/火箭/...)
1.3 数据处理
  1. 进行意图识别过程：根据 issue title + body 分类意图，目前主要将意图分为：
    1. \textbf{Technical Support (主要是为了筛选这类意图的 issue，适合改写成问题）}
    2. Bug Reports 
    3. Feature Requests 
    4. Documentation Updates 
    - 意图分类 Prompt：
    
issue_intent_prompt = """\
�� GitHub Issue Classification Assistant ��

I'm here to help you classify GitHub issues into predefined intent categories. 
Please provide the issue details, repository name, and programming language below, and I'll analyze them to determine the most appropriate category.

Intent Categories:
1. ❓ Technical Support or Troubleshooting: Requests for assistance, questions, or clarification regarding the project.
2. �� Bug Reports: Issues reporting errors, anomalies, or unexpected behavior in the software. 
3. ⭐ Feature Requests: Proposals for new features or enhancements  to the existing functionality. 
4. �� Documentation Updates: Suggestions for improving the documentation, fixing inaccuracies, or clarifying explanations.
5. �� Miscellaneous: Issues or discussions that do not fall into the above categories.

Please provide the following details:

Repository Name: [repo_name]
Programming Language: [repo_language]

Issue Title: [issue_title]

Issue Description:
[issue_description]

I'll analyze the provided information, taking into account the repository context, and classify the issue into one of the intent categories. I'll provide the classification results in the following format:

Classification Results:
- Category Number: [1-10]
- Category Name: [Category Name]
- Explanation: [Brief explanation of the classification reasoning]

Example Response Format:
Classification Results:
- Category Number: 1
- Category Name: �� Bug Reports
- Explanation: The issue describes an error that occurs when trying to save a file, indicating it is a bug report.

Now, please provide the real details for issue classification.
Repository Name: {repo_name}
Programming Language: {repo_language}

Issue Title: {issue_title}

Issue Description:
{issue_description}

Classification Results:
"""


2. Query 处理：LLM 改写 Issue title + body，把 issue 改成一个较为简单合理的 query，符合用户直觉上会在侧边栏提问的问题。
- Query 改写 Prompt 如下：


transform_issue_prompt = """
GitHub Issue to User Question Assistant ��

I will assist you in transforming a GitHub issue into a question that a user might ask a language model. Please provide the issue title and body, and I will analyze the content to generate a question representing the user's query. If the issue contains small code snippets, I will try to preserve them as much as possible.

Repository Name: [repo_name]
Issue Title: [issue_title]
Issue Description:
[issue_description]

Based on the GitHub issue above, I have generated the following user question:

Transformed User Question: [use_question]

This generated question aims to capture the core points of the original GitHub issue in a clear and natural way, representing a user seeking help or guidance from the language model. If the issue contained code snippets, I have tried to preserve them in the generated question to the best of my ability. If you have any other GitHub issues you'd like to transform, please feel free to provide them to me.
Please provide the repository name, issue title, and description to continue.
Repository Name: {repo_name}
Issue Title: {issue_title}
Issue Description:
{issue_description}

Transformed User Question: \
"""


3. Answer 处理：LLM 根据 issue title，issue body，改写的query，生成参考答案
- Final 数据格式: [query, query_intent, comments, answer_points, issue_url, issue_title, issue_body, latest_commit_hash]
- Answer 获取 Prompt:

    
summarize_issue_prompt = """
GitHub Issue Answer Generator ��

I will provide a direct answer to help resolve a GitHub issue, based on the issue comments, issue body, issue title, and a summarized question.
The helpful information is extracted from the issue comments and combined with the summarized question to generate a clear and actionable answer. 
I will focus on the issue comments that have received the most positive feedback (e.g. "+1", "rocket", "hooray" icons), as they likely contain the most helpful information.

Repository Name: {repo_name}
Issue Query (question to be answerd):
{summarized_question}
Issue Title: {issue_title}
Issue Description:
{issue_description}

Relevant Information from Issue Comments:
{issue_comments}

The issue answer aims to provide a clear, actionable solution or recommendation to resolve the GitHub issue, by synthesizing the most relevant and positively received information from the issue comments, title, description, and the summarized question. The goal is to directly address the core problem and provide useful guidance to the issue reporter and others who encounter the same challenge.
When generating the answer, please follow these guidelines:
- Summarize the key points and steps from the relevant comments without attribution.
- Prioritize clear, actionable recommendations that directly address the issue.
- Focus on providing a general solution without mentioning specific users.
- Present the solution directly, without mentioning the source of the information, specially, don't mention this solution from issue.

Issue Answer: \
"""


4. 人工看数据 & 筛选出高质量的 qa pair
TODOS
  [] 对于有代码生成（如：代码修改/Feat/Fix...）的任务，采用 SWE-bench 的方式收集 or 自己爬到对应的 file changes，使用通过测试用例个数评估
    - Final 数据格式: [query, query_intent, file-changed/test-passed, , issue_url, issue_title, issue_body,  latest_commit_hash]




==> materials/dataConstructionPipeline.tex <==


1. 从四种语言（Python, Java, Go, TypeScript） 爬取 TOP 500 的仓库 ==> 2000 仓库

仓库选择



1.1 从爬取的仓库中，筛选 (closed issue+pulls 数)>1000 &  <50000 的仓库 & public &  可以被爬取的（有valid licenses） ==> 890 仓库
1.2 我们从其中根据预估的仓库数量的大小，对于每个语言，随机挑选 5 个支持 long context evaluation（预估 token 数量 < 200K ）其中 java 只有 3个。
随机挑选 50 个 > 200K的仓库。
1.3  总共 \textbf{218} 个仓库，共有 1623624  Issues + Pulls（因为 Github API isssue 和 pull 用的是同一个） 

issue 爬取 
爬取所有仓库 Issues with comments，总共爬到了 1580208 个 Issues + Pulls（TBD：这个数字可以不说？）

issue 规则过滤
根据过滤规则过滤掉 issues，规则如下：
0. 是 Issue 不是 Pull（TBD：不说？）
1. issue tag 中没有 feat, bug, fix, error（因为这些需要 Fix 的内容往往不会给出直接有效的答案，和 PR 联系在一起，模型很难从对话中总结出解决方案）XX
2. issue body 中没有图片（确保用户描述的问题模型不会MISS）XXX
3. issue body 中有 ``` 包裹的代码片段（这些代码片段，可以最为转化的问题的参考信息）
4. issue comments 中至少有一个 comment 是至少包含 K 个(K=3) 正向反馈的 comment，且这个comment 中没有 url 信息（这样确保模型答案不会让用户再去check xx url）.
4.1 至少有一个 comment 是至少包含 K 个(K=3) 正向反馈
4.1.1 且 没有 url 

这一步骤最终获得了 \textbf{8977} 个 issues，包括在 213 个仓库里面


从每个仓库中（如果多于300个issues）随机挑出 300 个Issues， 得到 4306 个issues(213repo)


issue llm 分类过滤
让 LLM 判断 Issue 是否是一个 可以转化成好的QA问题的 Issues。如果不是，则过滤掉。
得到2127 issues/ 190 repo


build QA 数据集
目前总共问题 \textbf{1757}  (有些Issue Query/Answer FinalPrompt (卡最长 Token = 30000)太长了，回答不了)，这个最终可以 说下我们挑出了一些题生成了问题



QA后处理
后处理
1. 筛选出回答中没有 ‘version xx’ 的 issues（一般这个需要很多version的信息，质量比较差）原因：XXX
2. 给每一条 QA 数据记上 latest Commit information


1702题目，180个仓库

人工筛选(TODO?)
-  QA 数据集质量究竟如何？
5个人 sample 了500题，每人 200题，每一题都有两个2个人的结果。。
1. 对于每一条数据，点击列 issue-html-url，打开网页
2. 根据 【网页｜ query列 ｜ reference-answer 列】，逐步检查
  1. 根据打开的 issue 网页中的 issue-title 和 issue-body，首先检查这个 issue 是否提出了一个有效的仓库的代码问答题目，这个 issue 的问题的质量高不高。
  2. 检查由issue title 和 body 改写成的 Query 列是否完全表达了 issue 提出者的意思，改写 query 是否有问题
  3. 根据 issue 网页中的点赞/其他正向评论 issue-comments，检查 reference-answer列是否正确表达了 issue-comments 的意思
  4. 检查 reference answer 的质量，是不是对上述改写的 query 一个直接有效的的回答，而不是让用户去看其他内容获取答案
3. 根据上述检查流程，给这条数据打分 【0 - 5】分
  1. 如果不是有效的仓库代码问答题，直接打 0 分
  2. 如果回答是间接且模糊的，直接打 0 分
  3. 其他情况，酌情打分 【1，2，3，4，5】

召回相关信息
1. Checkout 到指定 Commit
2. 使用 LangChain Splitter 切分仓库
3. 使用 BM25 召回信息（分别使用 query，answer，issue body 中的 code snippet 召回信息） 

最终数据字段有
- query, issue-body-code-snippets
- reference-answer
- repo-url, repo-language
- issue-html-url, issue-create-time
- lastest commit sha before create time
- top10 bm25 retrieval chunks from query
- top10 bm25 retrieval chunks from reference-answer
-top10 bm25 retrieval chunks from issue-body-code-snippets

TODO数据集分析？
1. check 一下，每个仓库 2024 January 前、后 各多少问题？
issue\_create\_time 
2012 3 
2013 4 
2014 22 
2015 76 
2016 143 
2017 170 
2018 288 
2019 269 
2020 324 
2021 157 
2022 97 
2023 123 
2024 26

2. 每个语言都有多少条数据？
language distribution 
TypeScript 573 
Python 507 
Go 397 
Java 225

3. 小于 190K 的issues 数量有多少，涉及多少个仓库？（留出一些给问题和system prompt）
(96,) 个issue， 涉及   10 个仓库

获取模型回答
1. DONE 跑出 4 个模型没有召回信息的回答

2. running 跑出加上 TOP5 Query 召回 + TOP5 Query 代码召回的回答
（数据集提供了 answer 召回的回答, 召回过程不用）

3. DONE Long Context Model Prompt 获取模型回答

获取绝对值打分结果
1. RUNNING 获取没有召回信息的打分结果，重新搞下打分 Prompt，之前的Prompt 不是特别准确

获取相对打分结果
TODO




---- 应该可以不用了 ---- 最新版本质量还可以
QA  筛选
Prompt 设计 + QA 过滤
给 QA 数据集质量标注，过滤掉质量低的








  

-------------------------------------------------------



最终选出得分较高的题目，保留～2000 个问题

选出题目后，跑模型回答，
1. 调通所有模型的 API
2. 构建好所有 Final Prompt
[]模型需要用 召回信息
[]模型需要用 repo2text 方法（代码在 utils.repo_to_text.py)

打分策略
[]绝对值打分 2000 * 3（次）
[]对比打分（这个是否太耗时间）
        2000 * 3 * C_n^2
[] 结果统计






final_score
5    7183
4     644
3     324
0     313
2      59
1       5


---------------------------------
issue_create_time
2011       1
2012       4
2013      18
2014      42
2015     181
2016     503
2017     756
2018    1005
2019    1025
2020    1282
2021     948
2022     718
2023     744
2024     228




==> materials/refine_prompt.tex <==

You are an professor on software engineering and natural language processing for over 20 years. I'm writing a paper to release a benchmark for code repository question answering which is a leading natural language processing and software engineering academic journal. In this chat, you need to help me refine my representation. If I input in Chinese, you need to translate it to English first. Try to understanding what I want to express and refine it for clarity, coherence and conciseness, ensuring each paragraph flows into the next. Remove jargon. Use a professional tone. 








==> materials/sketch_V0.tex <==
% 商业产品 + 学术Citation高 open code + 对比延迟和效果

% 前面的bench构造过程描述可以参考下 CodeAgent: https://arxiv.org/pdf/2401.07339.pdf

% \section{Introduction}
% CodeQA 数据集就很缺失。
% 先总结现状：Code understanding / comprehension 怎么实现的
% 要提到的点：
% - 先总结目前的 Benchmark：其中一个结论是benchmark 大部分是简单任务。如 HumanEval 等
% - 然后，介绍目前的趋势就是在做 “难任务”，需要更复杂的评测。这里先提到现在做 Repo-level Tasks 的一些方法： RepoCoder 等paper。再此基础上介绍一些 Repo-level bench，比如 RepoBench、CrossCodeEval 总结这些数据集大部分都在做 Code Generation。而我们做 QA。
% - [WIP] SWE-Bench 着重讲一下 SWE-bench ,xxx 等，SWE-bench 更面向解决问题（ Add a feature, Fix a bug ）SWE-bench 的弊端有：1.目前只有Python 语言。
% - 从而引出，RepoQA bench 目前是缺失状态，没有一个好的benchmark 来衡量 RepoQA System。类似的有21年的一篇文章 CodeQA （太简单了），所以我们做了基于 Issue 的 RepoQA。



%%%%%%%

% 先确认一个问题：数据集 衡量需要配合 RAG 
%   - 理由：没有 Repo 额外的信息，Issue 问题基本无法被回答。【需要一个实验/比率】
% 红色部分需要仔细讨论


% 1. Introduction



% main contributions:
% 1. RepoQA 数据集构建过程。数据的质量，统计信息。确定benchmark。
% 2. 在数据集上进行了 xxx 实验。xx 模型 + xx 召回策略得到了 xx 结论。 
% 3. 长文本模型评测？

% 2. RepoQA Benchmark
% 2.1 Datasets Construction
% RepoQA Eval Datasets
% 1. 先介绍 Formats & Example
% 2. Data 收集处理过程:
%   - 数据收集： 
%     - 仓库选择：是否需要按照语言，token 数量，选择 
%       - TODO: 仓库确定 需要看 Repo-mining相关
%       - 参考 DEV-Bench 仓库选择方式  （20个仓库 4个语言
%       - 包含语言：Python / Java / Go
%       - 每种语言仓库大小分布： XXX 
%       - 仓库的领域：AI / 前端 / 后端 ?
%     - 爬取哪些数据？Issue with comments
%   - 清洗处理过程： 
%     - 不要和 PR 关联的数据 (确保不和 SWE-bench 冲突）
%     - 有点赞的 comments
%     - xxx 过滤策略 （需要完善）
%   - Issue 改写成 Query
%     - Prompt 实验是否需要做 Ablation？
%     - <Issue body + Issue title, Repo-metadata, Prompt, LLM> → query
%     - 专家+人工评审 ,issue
%   - Comments 改写成 Answer
%     - Prompt 实验是否需要做 Ablation？
%     - <Issue body + Issue title, Query, Repo-metadata, Prompt, LLM> → answer
%   - ? 召回信息 （这个怎么构建 Golden 召回？） 
%     - 先用 CKG 召回20个，再人工筛选，宣称是人类专家得到
%     - 从 query 构建还是从 answer 构建，or 其他方法？
% 3. 数据验证 verfication ？这个数据集为什么质量高
%   - 参考 DEV-bench （人类和模型的结合方式）

% 2.2 Datasets Characteristics & distributions
% 多少仓库？多少个问题？问题分类？Examples？

% 2.3 Benchmark Evaluation Procedure
% 先说各个评价指标，再说评估流程
% Evaluation Metrics for this datasets
% 感觉评价指标和 RAGAs 那篇文章的评价指标比较像
% - Relevance between <Query, generated_answer>(Embedding Cosine Similarity)
% - Similarity between <ref_answer, generated_answer> (Embedding Cosine Similarity or Bleu Score)
% - Correctness 
%   - LLM as scoreler
%   - Input = Prompt + Query + Generated_answer + CodeSnippets)
%   - 多次取平均？
% - Latency

% \section{Empirical Study (Experiments)}

% \subsection{RQ1. LLMs 在这个数据集上表现咋样？}
% RQ2. 不同的 RAG 方式对结果的影响？
% RQ3. 直接用整个REPO + 长文本模型的表现如何？（没人做过）
% RQ1. Evaluate performance of product & tools 
% Exp setup：
% Products:
% - 公司产品：Phorm, Cursor, Copliot Chat
% - LongContext：Gemini1.5Pro Claude3-Opus-200K Kimi-200
% 预期结论：xx 模型比较好

% RQ2: Long Context
% - LongContext：Gemini1.5Pro, Claude3-Opus-200K, Kimi-200

% RQ3: Products VS Longcontext

% RQ4: Latency


% RQ2. Evaluate RAG system (召回策略):
% 实验 setup:
% - 同一个基础模型 with 不同的召回策略： GPT4 
%   1. BM25？
%   2. 文本切分 + Embedding ？
%   3. RepoCoder 的方法？
%   4. RepoAgent ?
% 预期结论：xx 召回方法有效。

% RQ3. Evaluate RAG vs Long Context Model
% Exp Setup:（用RQ2最好的方法）
% - Gemini 1.5 + Fullrepo
% - Gemini 1.5 + RAG Info
% - Claude3 + Full repo
% - Claude3 + RAG Info
% 预期结论： RAG 和 LongContext 哪个有效？延迟？
% 4. Related work
% 主要会议：ICSE / ICLR / 
% 数据集：
% https://github.com/saltudelft/ml4se?tab=readme-ov-file#datasets
% - CoderEval
% - RepoBench
% - SWE-bench
% - ClassEval
% - Effibench
% - CodeComplex
% - DS-1000
% - XCodeEval
% - CrossCodeEval
% - HumanEval
% - HumanEval+ 
% - RealHumanEval
% - CodeQA
% - CodeScope
% - Devbench
% - CRUXEval
% - ...
% Repo-level code tasks
% - When Large Language Models Confront Repository-Level Automatic Program Repair: How Well They Done?
% - Repository-Level Prompt Generation for Large Language Models of Code
% - RepoCoder: Repository-Level Code Completion Through Iterative Retrieval and Generation
% - CodePlan: Repository-level Coding using LLMs and Planning
% - CodeAgent
% - Repoformer
% - ...

% 5. Conclusion
% - discussion: 这种数据，搭配上 RAG 召回的信息，是否可以作为 SFT 数据？

% Future work


% THREAD MODEL
% - 现在是模型打分，之后xxx
% - 
% Refs
% - https://arxiv.org/abs/2306.05685 NeuraIPS 2023
%   LLM as a judge(背书论文）Judging llm-as-a-judge with mt-bench and chatbot arena. arXiv preprint arXiv:2306.05685, 2023a.
%   - 结论：模型和人类评估可以达到类似的水平。strong LLMs can achieve an agreement rate of over 80%, on par with the level of agreement among human experts, establishing a foundation for an LLM-based evaluation framework.
% - https://github.com/lm-sys/arena-hard/tree/main
%   - Following LLM-as-a-Judge and AlpacaFarm, we employ LLM as a judge framework to approximate human preference.
%   - arena-hard https://lmsys.org/blog/2024-04-19-arena-hard/
% - https://arxiv.org/pdf/2109.07958.pdf TruthfulQA  -- 简单 QA 数据集
%   - 它的做法：每个Q 提供 True False 两个答案集合，以及一个证明True的相关资料
%     - Each question has sets of true and false reference answers and a source that supports the answers (e.g. a Wikipedia page) 


==> todos.tex <==
 % 1. 可能计算下：QA 占所有问题的比率，
% 2. 我们收集的issues的平均 word 长度




\section{TODO}

\textbf{abstract ddl: 26 July 2024. 
submission: 2 Aug 2024}

\textbf{Target}: ICSE'2025 - Research Track - \textit{Efficacy measurement beyond traditional metrics (e.g., accuracy, BLEU, etc.)}


\begin{CJK}{UTF8}{gbsn}




\textbf{结果统计}:
\url{https://docs.google.com/spreadsheets/d/1R1QzBs0huxzSkU4DpGgXX-kE7n130PW_7ZW4mKwB47I/edit?usp=sharing}

\subsection{Discussion: 2024/06/20}

\textbf{期望 6.30前完成所有实验，}

需要讨论内容

1. 代码： 

2. issue + comments 

3. 模型选择： gpt4o, deepseek v2, claude3, genimi1.5 

3. 实验排期Table~\ref{tab:main_results}

    3.1 仓库收集： 
        
        top 500 ； 2024/06/18 收集的 

        TypeScript, GO: jiangliang

        Python, JAVA: kaifa

        
        
        
    3.2 issue 筛选：

        issues 全爬下来再过滤

        
    3.3 query + answer 生成：


    3.4 评估：


4. pairwise evaluation 评分记分



CONFIRM：
1. 先把issue -> QA 流程打通，实验做完； discussion，之后再加
2. 




\subsection{Discussion: 2024/06/16}

1. 公开内容： 

1.1 < Question, Answer, RepoURL\&Commit, Issue ID, Retrieval Information（文件级别） >

1.2 评估框架/系统 



2. 实验设置

2.1 模型：

2.2 评估次数：



3. 样本：

以 1.1 为例，给个example，写到对应章节


4. 评估框架细节:

4.1 如何设计的，每一步设计的思路的是什么，为什么这么设置


\subsection{Discussion: 2024/05/29}
1. 意图选择： 保证生成的 Query 在流程上、验证上都是Repo相关的

2. 数据量：X个语言， Y 个仓库， K 题 = X * Y * K

3. 评估器/评估平台设计： 我们是QA，Ans 一般为自然语言+code snippets。即便我们生成答案的过程有可信参考 + 专家标注，也需要考虑如何使我们的评测集不仅可信，而且方便用户使用。

4. 

\subsection{TO Confirm 2023/06/08}
% \jialiang
% \kaifa{麻烦 @jialiang 大佬把这块细化一下不？}
比如：我们怎么选择的仓库：
\jialiang{仓库选择逻辑update到了仓库中}
\jialiang{https://github.com/cjl99/repoqa-dataset 可能需要加权限}
\textbf{1.} 先确定语言：Python, Java, GO (C, C++, Kotlin, TypeScript, JavaScript, Rust)


\jialiang{ 目前只做了主流的4种语言： Python, Java, Go, TypeScipt }

\textbf{2.} 针对每个语言选择 TOP XXX 的仓库（TOP 怎么确定，根据 Star、comments数 数还是什么)

\textbf{2.1} 过滤掉哪些仓库，比如总代码行数大于多少的不要，或者 repo zip size 大于多少的不要， 没有 comments 的不要等等
\textbf{2.2} 还是选择 有 issue 的仓库？ 对fork 什么的又没有过滤等

\jialiang{过滤操作具体在代码中有，需要讨论的
1：我觉得还需要额外的仓库筛选步骤（最热门repo是教学类的）
2: 什么是popular 的仓库，仓库筛选需要 ref
}
\kaifa{1. 教学类没太大问题
2. 以 stars 数 为标准即可}


\textbf{3.} Issue with comments 选择： 使用 GitHub api？ 选择 open/close issues with comments?
 	\textbf{3.1} issue 是否需要过滤，如何过滤，为什么这么过滤
\jialiang{yes， 目前的过滤逻辑是
1.通过模型筛选出 ‘seeking for help’ 的issue。 
2.选出2024.1.1后（目前做了一些实验感觉这个还存在问题，太少了（之前我记得讨论是改写后的query/answer应该不会过多的影响效果。如果2024.1.1后的太少我们是不是可以开源两个版本的数据集（1个所有时间，1个xx后）。 
我的代码可能需要改成先把所有 issue都爬下来然后再进行筛选。这样可以防止重复工作，现在为了节约时间只爬下来了 2024.1.1， 3.有comments）}
\kaifa{
for 2. issue 可以 2024.1.1 前后各占50\% 便于之后加一些对比实验； 需要都爬下来，即便不爬下来，可以统计下：目标仓库有多少issues (issue number, IN), 我们过滤了多少，最后有多少 final number FN，最后又一个比率 IN/FN 都可以写
}
 	\textbf{3.2} comments 过滤 
 		\textit{3.1.1} 有点赞的comments， 如何过滤（使用github api？还是规则？）
\jialiang{目前的逻辑都在代码中。遍历所有comments}
 		\textit{3.1.2}  



\textbf{4.} Issue 改写 query
	\textbf{4.1} 目的： 使得生成的 comments 更真实， 使得 query 更像用户会使用的问题
	\textbf{4.2} 方法： 使用prompt + llm，使用了哪些技术，给个例子如果ICL的话给个例子，例子如何来的
\jialiang{Prompt目前放在代码中，需要kaifa大佬review提意见}
\textbf{5.} Comments 改写answer： 
	\textbf{5.1} comments 是否需要过滤 
	\textbf{5.2} 目的：使得参考答案有据可依
	\textbf{5.3} 方法： 使用prompt + llm， 使用了哪些技术，
		TODO： 这些 comments 是否作为 RAG 的一部分？如何确定，

\textbf{6.} Retrieval information： 理论上回答我们的问题肯定需要 cross-file reference 如何确定这些信息；怎么加到我们数据集的生成过程中比较合理，大佬怎么实现的可以歇一下

\textbf{7.} 参考答案的生成似乎是仅依赖 issue + comments 的，代码仓库相关信息是何时给出的，如何给出
\jialiang{我目前想法是使用 Langchain 的代码切分逻辑 + Embedding 召回}



\textbf{8.} 需要一个github comments的case
\jialiang{WIP 正在挑选中，之后我觉得需要放两个case一个来自issue一个来自dicussion}

\end{CJK} 


\begin{comment}
    

\subsection{Discussion: 2024/05/28}
@Kaifa @Jialiang

1. Why our dataset names RepoQA. Why repository information is necessary to answer the questions? % (从现在整理到的东西来看，这个结论似乎来自于我们的经验)
% 做数据集的原因，没有办法
% 不用 repo 信息，没有办法很好的回答这些问题；
% 我们选择 issue + comments 的时候必须会有


2. Will we provided reference information to answer the Questions?  \textbf{YES}
    2.1 If yes, could we provide automatic methodology to construct those information?
      TODO \textit{BM25}  + \textbf{expert label/filter}
    
    
3.\begin{CJK}{UTF8}{gbsn}
从现在来看，我们的主要有趣的点在于
3.1. Query 的构造，相当于是issue 相关的 （这里是不是 说因为直接用issue 问 llm 无法得到有效的回答，也许需要做一个 exp 说明），
3.2. answer 的构造是基于 issue + comments ， 相当于我们答案的生成有依据， 但并不能说明它可靠？
    1. 评估流程上做优化，
    2. 人工/专家check
\end{CJK} 
    
\end{comment}


% 1. The repositories in SWE and CodeAgentBench both select repository with self-contained test suites.



% 下次讨论： 
% 1. 分类出意图的数据做筛选
